A Survey on Image Aesthetic Assessment

Automatic image aesthetics assessment is a computer vision problem dealing with categorizing images into different aesthetic levels. The categorization is usually done by analyzing an input image and computing some measure of the degree to which the image adheres to the fundamental principles of photography such as balance, rhythm, harmony, contrast, unity, look, feel, tone and texture. Due to its diverse applications in many areas, automatic image aesthetic assessment has gained significant research attention in recent years. This article presents a review of the contemporary automatic image aesthetics assessment techniques. Many traditional hand-crafted and deep learning-based approaches are reviewed, and critical problem aspects are discussed, including why some features or models perform better than others and the limitations. A comparison of the quantitative results of different methods is also provided.

==> sections-plos/AuthorContributions.tex <==
\section*{Author Contributions}
\begin{itemize}
    \item \textbf{Conceptualization}: Abbas~Anwar, Saira~Kanwal, Muhammad~Tahir, Muhammad~Saqib, Muhammad~Uzair.

\item
\textbf{Data curation}: Abbas~Anwar, Saira~Kanwal, Muhammad~Saqib, Muhammad~Uzair.

\item
\textbf{Formal analysis}: Abbas~Anwar, Saira~Kanwal, Muhammad~Tahir, Muhammad~Saqib, Muhammad~Uzair.

\item
\textbf{Methodology}: Abbas~Anwar, Saira~Kanwal,  Muhammad~Saqib.

\item
\textbf{Project administration}: Muhammad~Tahir, Muhammad~Saqib, Muhammad~Uzair, Mohammad~Khalid~Imam~Rahmani.

\item
\textbf{Supervision}:  Muhammad~Saqib, Muhammad~Uzair, Muhammad~Tahir.

\item
\textbf{Funding acquisition}: Muhammad~Tahir, Mohammad~Khalid~Imam~Rahmani.

\item
\textbf{Resources}: Abbas~Anwar, Muhammad~Saqib, Muhammad~Uzair.

\item
\textbf{Visualization}: Abbas~Anwar,  Muhammad~Saqib, Muhammad~Uzair.

\item
\textbf{Writing - original draft}: Abbas~Anwar, Saira~Kanwal.

\item
\textbf{Writing - review $\&$ editing}: Abbas~Anwar, Saira~Kanwal, Muhammad~Tahir, Muhammad~Saqib, Muhammad~Uzair, Mohammad~Khalid~Imam~Rahmani.

\end{itemize}



==> sections-plos/keywords.tex <==
\begin{IEEEkeywords}
Image aesthetic assessment, feature extraction, classification, convolutional neural networks, deep learning
\end{IEEEkeywords}
